Learning to Model the Grasp Space of an Underactuated Robot Gripper Using Variational Autoencoder

Grasp planning and most specifically the grasp space exploration is still an open issue in robotics. This article presents a data-driven oriented methodology to model the grasp space of a multi-fingered adaptive gripper for known objects. This method relies on a limited dataset of manually specified expert grasps, and uses variational autoencoder to learn grasp intrinsic features in a compact way from a computational point of view. The learnt model can then be used to generate new non-learnt gripper configurations to explore the grasp space.

==> input_output_table.tex <==
\footnotesize
\setlength\tabcolsep{5 pt}
\begin{tabular}{| *{12}{>{\centering\arraybackslash}m{0.34cm} |}}
\hline
\multicolumn{12}{|c|}{inputs} \\
\hline
\multicolumn{8}{|>{\centering}m{2.72cm + 14\tabcolsep + 2.8pt}|}{gripper configuration in frame $F_{obj}$} & \multicolumn{4}{>{\centering}m{1.36cm + 6\tabcolsep + 1.2pt}|}{tabletop plan cartesian equation in frame $F_{obj}$} \\
\hline
%\multicolumn{3}{|c|}{position} & \multicolumn{4}{c|}{orientation} &  & \multicolumn{4}{c|}{equation coefficients} \\
%\hline
$x$ & $y$ & $z$ & $q_x$ & $q_y$ & $q_z$ & $q_w$ & $\theta$ & $a$ & $b$ & $c$ & $d$ \\
\hline
\multicolumn{8}{|c|}{outputs} & \multicolumn{4}{c}{} \\
\cline{1-8}
\end{tabular}
